ElasticDiT: Efficient Diffusion Transformers via Elastic Architecture and Sparse Attention for High-Resolution Image Generation on Mobile Devices

The Diffusion Transformer (DiT) architecture is the state-of-the-art paradigm for high-fidelity image generation, underpinning models like Stable Diffusion-3 and FLUX.1. However, deploying these models on resource-constrained mobile devices entails prohibitive computational and memory overhead. While efficiency-driven approaches like Linear-DiT and static pruning alleviate bottlenecks, they often incur quality degradation. Unlike cloud environments, mobile constraints require a single-model paradigm that dynamically balances fidelity and latency. We introduce ElasticDiT, which achieves this dynamic trade-off by adjusting spatial compression ratios and DiT block depths. By integrating Shift Sparse Block Attention (SSBA) and a Tiny DWT-Distilled VAE (T-DVAE), ElasticDiT reduces inference latency and memory footprint while maintaining image quality. Experiments confirm that ElasticDiT effectively covers a wide range of fidelity-latency trade-offs within a single set of parameters. By jointly adjusting compression and depth, a single ElasticDiT model can be reconfigured on-the-fly to outperform task-specific baselines. Specifically, our flex lite variant achieves an HPS of 32.87, surpassing the Flux model, while maintaining competitive quality at 84.16 percent average sparsity through SSBA. Furthermore, the plug-and-play T-DVAE provides SD3-level reconstruction with only 1/8x the computational cost of standard VAEs, and Flow-GRPO boosts semantic alignment (GenEval: 66.93 to 73.62). These results demonstrate that ElasticDiT offers a versatile, hardware-adaptive solution that eliminates the need for multiple specialized models, providing a promising path for future high-resolution image generation on mobile devices.

==> sections/1_introduction-manuscript.tex <==
\section{Introduction}
\label{sec:intro}

Diffusion models have reached a generative-AI inflection point where photorealistic fidelity and open-vocabulary semantics are simultaneously attainable within a single framework. Over the past year, Stable Diffusion 3 and Flux have pushed parameter counts from billions to tens of billions by replacing the U-Net backbone with the Diffusion Transformer (DiT), unleashing unprecedented visual quality and fueling a surge of downstream tasks such as image super-resolution and semantic editing.

Yet when these powerful models are migrated from cloud GPUs to memory-constrained edge SoCs, the same ``megapixel leap'' becomes a quadratic cliff: doubling the spatial resolution quadruples the self-attention cost.  
Two algorithmic escape routes have emerged---sparse or linear attention to curb FLOPs, and weight pruning/quantization to shrink memory.  
Unfortunately, any rigid reduction in compute budget irreversibly trades high-frequency texture or semantic alignment, culminating in artefacts most perceptible to mobile users: blurred text, erased pores, and object boundaries that drift from the prompt.

By re-dissecting this bottleneck, we find that the root cause is not ``insufficient compression'' but ``representation over-provisioning.'' At every denoising step, low-frequency global semantics permanently occupy memory, whereas high-frequency details only need to be referenced accurately in a few steps, yet both are processed through dense operations throughout. Hence, ``deciding what not to compute'' unlocks more edge-side efficiency than ``making the remainder cheaper.''

Driven by this insight, we present \textbf{sDiT}, a diffusion Transformer natively architected for edge deployment.  
Instead of treating efficiency as an after-market retrofit, we bake sparsity and elasticity into every layer:
\begin{enumerate}
	\item \textbf{Swin 2D Sparse Attention.} We introduce a novel window-based sparse attention that retains global receptive fields while locking complexity to linear growth.  
	\item \textbf{Shared-Weight Multi-Scale Base Model.} A single set of weights equipped with switchable skip-layer paths instantiates either a 1.3 B high-fidelity mode or a 0.6 B rapid mode without redundant storage. 
	\item \textbf{Multi-Stage VAE Distillation.} A wavelet-guided distillation pipeline compresses VAE latency by 4$\times$ and memory by 8$\times$ while preserving pixel-perfect reconstruction.
\end{enumerate}

sDiT breaks the ``compress$\rightarrow$degrade$\rightarrow$recover'' cycle: one checkpoint generates 4 K posters on premium tablets and delivers 1024$\times$1024 wallpapers in $<$1s on entry-level phones, while CLIP-I and FID remain on par with cloud-scale baselines. We expect sDiT to set a new on-device generative baseline---where high resolution, high quality, and high flexibility are no longer tethered to a power cord.

%扩散模型已抵达生成式AI的关键拐点：在一个框架内同时实现照片级逼真度与开放词汇语义。过去一年，Stable Diffusion 3 和 Flux 把参数量从十亿级推到百亿级，用 Diffusion Transformer（DiT）替换 U-Net 骨干，带来前所未有的视觉质量，并引爆超分、语义编辑等下游任务。
%然而，当这些强大模型从云 GPU 迁移到内存受限的边缘 SoC 时，同样的“百万像素飞跃”却变成二次方悬崖：空间分辨率翻倍，自注意力开销就近乎四次方暴涨。
%目前两条算法逃生路——稀疏或线性注意力砍 FLOPs，权重剪枝/量化压内存——都过于刚性：算力预算一旦削减，高频纹理和语义对齐就不可逆地受损，最终把最刺眼的artifact留给手机用户：文字发糊、毛孔消失、物体边缘偏离提示词。
%重新拆解瓶颈后，我们发现根源不是“压缩得不够”，而是“表示过度供给”。每一步去噪里，低频全局语义始终占着内存，而高频细节只需在少数几步被精准引用，却同样全程经历稠密运算。因此，“决定不算什么”比“把剩下的算得更便宜”更能释放边缘效率。
%受此洞察驱动，我们提出 sDiT，一款原生为边缘部署设计的扩散 Transformer。效率不再是事后打补丁，而是把稀疏性与弹性烘进每一层：
%Swin 2D 稀疏注意力。新颖的窗口稀疏注意力在保持全局感受野的同时，把复杂度锁成线性增长。
%共享权重的多尺度基模型。同一套权重配合可切换的跨层skip路径，既能化身 13 亿参数的高保真模式，也能切到 6 亿参数的极速模式，无需冗余存储。
%多级 VAE 蒸馏。小波引导的蒸馏管线把 VAE 延迟压到 1/4，内存压到 1/8，仍保持像素级重建。
%sDiT 打破“压缩→退化→补救”的循环：一个检查点既能在高端平板上生成 4K 海报，也能在入门手机上 1 秒内吐出 1024×1024 壁纸，CLIP-I 和 FID 与云端大模型持平。我们期待 sDiT 成为新的端侧生成基线——高分辨率、高质量、高灵活性，不再被电源线拴住。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Text-to-image (T2I) diffusion models have achieved remarkable success in generating high-quality images from textual descriptions. However, their deployment in real-world applications is often hindered by significant computational challenges, particularly the quadratic complexity of self-attention operations and the substantial memory requirements for storing multiple model variants. These limitations become especially pronounced when targeting ultra-high-resolution generation (4K, 8K) or resource-constrained environments such as edge devices.

Recent advances have explored various strategies to address these bottlenecks. Sparse attention mechanisms, such as Mixture of Block Attention (MoBA) \cite{moba}, have demonstrated promising results in reducing computational complexity while maintaining model expressiveness. Similarly, efficient VAE designs have been proposed to reduce the computational overhead of latent space encoding and decoding \cite{bibid}. However, these approaches often require trade-offs between efficiency and generation quality, and typically necessitate maintaining separate model weights for different computational budgets.

In this work, we introduce sDiT, a unified framework that addresses these limitations through three key innovations. First, we propose Sparse Block Attention (SBA), which adapts the MoBA paradigm to 2-D latent spaces, achieving linear complexity while preserving global receptive fields through importance-driven block selection. Second, we design a multi-resolution skip-layer strategy with shared weights, enabling a single 1.3B parameter model to operate either as a full-power generator or as a 0.6B fast generator without storing redundant parameters. Third, we develop a lightweight VAE through tri-stage latent-aligned distillation, achieving 2-4× inference acceleration with minimal quality degradation.

Our comprehensive experiments demonstrate the effectiveness of these contributions. At 1024×1024 resolution, sDiT-0.6B surpasses Flux-12B in human preference scores while using 20× fewer parameters. The sparse attention mechanism achieves 84.16% average sparsity without degrading generation quality, establishing a new Pareto frontier between latency and fidelity. Furthermore, our distilled VAE maintains competitive reconstruction metrics while reducing latency by 2-3× compared to existing approaches.

These innovations collectively enable flexible deployment across diverse computational budgets, from real-time edge inference to high-quality cloud generation, using a single set of shared weights. Our code and models will be made publicly available to facilitate future research in efficient T2I generation.

%文生图扩散模型在“一句话出大片”上已屡创奇迹，却因两大顽疾难以落地：自注意力的二次方复杂度，以及“一生多”的权重冗余——每换分辨率或预算就得存一套新模型。当目标变成 4K/8K 超高清，或者内存抠到边缘设备级别时，这些问题被成倍放大。

%近期研究各显神通：MoBA 这类稀疏注意力用“块”代替“全图”，算力直线下降；轻量 VAE 也把编解码的耗时砍了一刀。然而它们大多在“效率—质量”天平上做单选题，且仍需为不同算力档位分别存模型，边缘端依旧吃不消。

%我们给出一次性解套方案 **sDiT**，只用“同一套权重”就能伸缩自如，核心有三板斧：

%1. **稀疏块注意力（SBA）**  
%把 MoBA 思想搬到 2-D 隐空间，图像 token 切成小方块，按重要性只算 Top-k 块，复杂度从 O(T²) 降到 O(T)，全局感受野却一块不落。1024×1024 生成里平均稀疏度 84 %，质量依旧在线。

%2. **共享权重的多分辨率跳层**  
%1.3 B 参数的“满血”主干自带“重要性感知”跨层短路，训练一次即可按需跳过 50 % 层，秒变 0.6 B 的“极速”模式，无需额外存参数，内存直接腰斩再腰斩。

%3. **三阶段隐空间对齐蒸馏 Tiny-VAE**  
%先让学生 VAE 的隐分布与老师对齐，再联合 L2+LPIPS+Patch-GAN 精雕解码， latency 再砍 2-4 倍，PSNR>31 dB、FID<2.3，像素级重建依旧稳。

%实验结果一句话：**1024×1024 生成，sDiT-0.6B 在人类偏好上反超 Flux-12B，参数却少 20 倍；4 GB 内存的边缘芯片也能跑 4K 图。** 从实时手机端到低延时云端，只需这一副“万能骨架”。代码与模型即将全开源，欢迎来卷。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Text-to-image (T2I) diffusion models have reached an inflection point where photorealistic fidelity and open-vocabulary semantics coexist in a single framework. By replacing U-Net with the Diffusion Transformer (DiT), recent works such as Stable Diffusion 3 (SD3) and Fluxhave scaled parameter counts to 12 B, unleashing unprecedented visual quality and powering downstream tasks from super-resolution to semantic editing.

Yet the ``megapixel leap'' becomes a quadratic cliff when these giants are migrated from cloud GPUs to memory-constrained edge SoCs.
Doubling the spatial resolution quadruples the self-attention cost: a single 1024$\times$1024 sample already exceeds 12 GB DRAM and 15 s on a mobile GPU.
Two algorithmic escape routes have emerged---sparse/linear attention to curb FLOPs and weight pruning/quantization to shrink memory.
Unfortunately, any rigid compute budget irreversibly trades high-frequency texture or semantic alignment, culminating in artefacts most perceptible to mobile users: blurred text, erased pores, and object boundaries that drift from the prompt.

Re-dissecting the bottleneck, we find that the root cause is \textbf{not ``insufficient compression'' but ``representation over-provisioning.''}
At every denoising step, \textbf{low-frequency global semantics permanently occupy memory}, whereas \textbf{high-frequency details only need to be referenced in a few steps}, yet both are processed through \textbf{dense operators} throughout.
Hence, \textbf{``deciding what not to compute''} unlocks more edge-side efficiency than \textbf{``making the remainder cheaper.''}

Driven by this insight, we present \textbf{sDiT}, a \textbf{sparsity-native} DiT family architected \textbf{from the ground up} for edge deployment.
Instead of treating efficiency as an after-market retrofit, we bake \textbf{sparsity and elasticity} into every layer:

\begin{enumerate}
	\item \textbf{Swin 2-D Sparse Block Attention (SBA).}
	We adapt Mixture-of-Block Attention (MoBA)~\cite{moba} to 2-D latent space.
	Image tokens are grouped into \textbf{non-overlapping 8$\times$8 blocks}; mean-pooled queries/keys produce a \textbf{block-level affinity matrix}, and a \textbf{top-$k$ gate} retains only \textbf{25\,\%} of blocks while keeping \textbf{full-resolution values} for detail preservation.
	A \textbf{shift-window schedule} alternates grid origins every layer, breaking partition artefacts with \textbf{zero memory overhead}.
	Complexity drops from $\mathcal{O}(T^2)$ to $\mathcal{O}(T_{\text{img}})$, enabling \textbf{4-K generation} on \textbf{4 GB RAM}.
	
	\item \textbf{Shared-Weight Multi-Scale Backbone.}
	A \textbf{single set of weights} is equipped with \textbf{importance-aware skip-layer paths} calibrated by SANA-style layer-saliency analysis~\cite{sana}.
	After a \textbf{four-stage co-training} recipe, the same checkpoint can be executed as either a \textbf{1.3 B high-fidelity mode} or a \textbf{0.6 B rapid mode} with \textbf{no redundant storage}, yielding \textbf{2$\times$ latency reduction} and \textbf{8$\times$ memory compression}.
	
	\item \textbf{Wavelet-Guided VAE Distillation.}
	We design a \textbf{Tiny-VAE} that replaces the mid-block attention with \textbf{multi-level Haar wavelet convolution}~\cite{wf-vae}.
	A \textbf{two-stage latent-alignment distillation} first matches the \textbf{Flux encoder's latent statistics} with pure L2 loss, then freezes the encoder and optimizes the decoder with \textbf{L2 + LPIPS + Patch-GAN} losses.
	The resulting decoder achieves \textbf{4$\times$ latency shrink} and \textbf{8$\times$ memory shrink} while preserving \textbf{PSNR $\geq$ 31 dB} and \textbf{FID $\leq$ 2.3} at 1024$\times$1024.
\end{enumerate}

To the best of our knowledge, \textbf{sDiT is the first T2I family that simultaneously achieves}
\begin{compactitem}
	\item \textbf{linear-complexity attention} without quality drop,
	\item \textbf{single-weight, switchable capacity} (0.6 B / 1.3 B),
	\item \textbf{4$\times$ VAE latency reduction + 8$\times$ memory compression} with \textbf{pixel-perfect reconstruction}.
\end{compactitem}
We expect sDiT to set a new \textbf{on-device generative baseline}---where \textbf{high resolution, high quality, and high flexibility} are \textbf{no longer tethered to a power cord}.

%文生图（T2I）扩散模型已来到拐点：照片级逼真度与开放词汇语义在同一框架里兼得。把 U-Net 换成 Diffusion Transformer（DiT）后，Stable Diffusion 3、Flux 等最新模型把参数量直接推到 120 亿，视觉质量史无前例，也带火了从超分到语义编辑的一众下游任务。

%然而，当这些“巨人”从云端 GPU 走向内存吃紧的边缘 SoC，“百万像素飞跃”瞬间变成“二次悬崖”：分辨率翻一倍，自注意力开销就近乎四倍——一张 1024×1024 样张在移动 GPU 上就要 12 GB 显存、15 秒才能跑完。  
%目前两条急救通道：稀疏/线性注意力砍 FLOPs，剪枝/量化压内存。  
%可惜，任何“硬预算”都会不可逆地牺牲高频纹理或语义对齐，最后全变成手机用户一眼看穿的 artifact：字糊了、毛孔没了、物体边缘跑偏。

%我们把瓶颈重新剖开，发现根因不是“压缩得不够”，而是“表示过剩”。  
%每一步去噪里，低频全局语义始终占着内存，高频细节其实只在少数几步被需要，却同样全程陪跑稠密算子。  
%因此，“决定不算什么”比“把剩下的算便宜点”更能给边缘设备松绑。

%带着这个洞察，我们提出 **sDiT**——一套“天生稀疏”的 DiT 家族，从第一行代码就为边缘落地而设计。效率不是事后打补丁，而是把稀疏与弹性烘进每一层：

%1. **Swin 2-D 稀疏块注意力（SBA）**  
%把 Mixture-of-Block Attention（MoBA）搬到 2-D 隐空间：图像 token 先切成不重叠的 8×8 块，用均值池化后的 Q/K 算块级亲和度，再经 top-k 门控只保留 25 % 块，而 Value 仍用全分辨率，细节不丢。  
%每层交替移位窗口原点，零显存开销即可打破切块 artifact。  
%复杂度从 O(T²) 降到 O(T_img)，4 GB 内存即可直出 4 K 图。

%2. **共享权重的多尺度主干**  
%同一套权重，配“重要性感知”的跨层短路，先用 SANA 式层显著性分析校准，再经四阶段协同训练。  
%一个检查点可秒切 13 亿参数高保真模式或 6 亿参数极速模式，零冗余存储， latency 直接减半，内存压缩 8 倍。

%3. **小波制导 VAE 蒸馏**  
%设计 Tiny-VAE：把原中间块注意力换成多级 Haar 小波卷积。  
%两阶段隐空间对齐蒸馏——先只用 L2 对齐 Flux 编码器统计量，再冻结编码器，用 L2+LPIPS+Patch-GAN 联合训解码器。  
%最终解码器 latency 缩 4 倍、内存降 8 倍，1024×1024 仍保持 PSNR≥31 dB、FID≤2.3。

%据我们所知，**sDiT 首个同时实现**：
%- 线性复杂度注意力，质量无损  
%- 单权重、可切换容量（0.6 B / 1.3 B）  
%- VAE latency 4 倍↓ + 内存 8 倍↓，依旧像素级重建

%我们希望 sDiT 成为新的端侧生成基线——高分辨率、高质量、高灵活，再也不用被充电线拴住。
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In recent years, text-to-image (T2I) generation has witnessed remarkable progress, with models such as Stable Diffusion 3 (SD3) and Flux leading the way. A major breakthrough has been the adoption of the Diffusion Transformer (DiT) architecture, which replaces the traditional U-Net, scaling models to billions of parameters (8B and 12B). This architectural shift has significantly improved generation quality, enabling a wide range of downstream applications like image super-resolution and editing, which have gained immense popularity.

%However, a critical challenge arises when deploying these powerful models to resource-constrained mobile devices. The computational complexity of the DiT architecture's attention mechanism scales quadratically with input resolution. As many downstream tasks require high-resolution outputs, often exceeding 1K, this quadratic growth leads to severe memory and latency constraints, resulting in a poor user experience on edge devices.

%To address this, prior works have explored various optimization strategies. Some have attempted to reduce the number of tokens by lowering the VAE's compression rate and replacing traditional attention with linear attention. While this approach effectively reduces computation, it often comes at the cost of a significant drop in image quality and fidelity, making it unsuitable for a wide range of photo-realistic applications on mobile platforms. Another line of research, inspired by the success of sparse attention in Large Language Models (LLMs), has migrated this technique to DiT and used fine-tuning to mitigate performance degradation. Similarly, works like SANA1.5 have explored model pruning, reducing a 1.6B model to 0.6B by evaluating the relative importance of DiT layers. This provides a trade-off between model size and performance, but for extremely memory-limited scenarios, deploying two separate sets of weights remains impractical and highly inefficient.

%This raises a fundamental question: Can we design a T2I model that is natively built for efficient and flexible on-device deployment while maintaining state-of-the-art image generation quality?
%In this work, we propose sDIT, a high-quality, edge-efficient T2I model designed from the ground up for on-device deployment. To overcome the memory and latency limitations of edge devices while supporting high-quality generation and flexible deployment, our core designs are as follows:
%Swin 2D Sparse Attention. We introduce a novel Swin 2D sparse attention architecture to handle the quadratic complexity of high-resolution inputs by leveraging window-based attention.
%Shared-Weight Multi-Scale Base Model. We propose a shared-weight, multi-scale base model with skip-connections, which allows a single set of weights to flexibly support various output resolutions, drastically reducing the memory footprint required for deployment.
%Multi-Stage VAE Distillation. We develop a multi-stage latent space alignment distillation method and introduce an efficient Discrete Wavelet Transform (DWT) operator, successfully compressing VAE latency by 4x and memory consumption by 8x.

%Our proposed sDIT model represents a significant step towards bridging the gap between high-quality T2I generation and practical, efficient deployment on resource-constrained edge devices.

